A Comparison of Functional Principal Component Analysis Methods with Accelerometry Applications

The association between a person's physical activity and various health outcomes is an area of active research. The National Health and Nutrition Examination Survey (NHANES) data provide a valuable resource for studying these associations. NHANES accelerometry data has been used by many to measure individuals' activity levels. A common approach for analyzing accelerometry data is functional principal component analysis (FPCA). The first part of the paper uses Poisson FPCA (PFPCA), Gaussian FPCA (GFPCA), and nonnegative and regularized function decomposition (NARFD) to extract features from the count-valued NHANES accelerometry data. The second part of the paper compares logistic regression, random forests, and AdaBoost models based on GFPCA, NARFD, or PFPCA scores in the context of mortality prediction. The results show that Poisson FPCA is the best FPCA model for the inference of accelerometry data, and the AdaBoost model based on Poisson FPCA scores gives the best mortality prediction results.

==> A comparison of functional principal component analysis methods with accelerometry applications/table1.tex <==

\begin{longtable}[t]{lll}
\caption{Characteristics of individuals included in the analysis}\\
\label{tab:1} \\
\toprule
  & Unweighted & Survey-weighted\\
\midrule
\cellcolor{gray!6}{Sample Size} & \cellcolor{gray!6}{1003} & \cellcolor{gray!6}{1003.00}\\
Number of Weekday (mean (SD)) & 4.55 (0.78) & 4.57 (0.76)\\
\cellcolor{gray!6}{Number of Weekend (mean (SD))} & \cellcolor{gray!6}{1.65 (0.60)} & \cellcolor{gray!6}{1.67 (0.59)}\\
Body Mass Index (\%) &  & \\
\cellcolor{gray!6}{\indent Normal} & \cellcolor{gray!6}{288 (28.7)} & \cellcolor{gray!6}{288.7 (28.8)}\\

\indent Underweight & 11 (1.1) & 12.3 (1.2)\\
\cellcolor{gray!6}{\indent Overweight} & \cellcolor{gray!6}{386 (38.5)} & \cellcolor{gray!6}{380.0 (37.9)}\\
\indent Obese & 318 (31.7) & 322.1 (32.1)\\
\cellcolor{gray!6}{Race (\%)} & \cellcolor{gray!6}{} & \cellcolor{gray!6}{}\\
\indent White & 606 (60.4) & 835.5 (83.3)\\

\cellcolor{gray!6}{\indent Black} & \cellcolor{gray!6}{196 (19.5)} & \cellcolor{gray!6}{75.6 (7.5)}\\
\indent Hispanic & 180 (17.9) & 65.6 (6.5)\\
\cellcolor{gray!6}{\indent Other} & \cellcolor{gray!6}{21 (2.1)} & \cellcolor{gray!6}{26.4 (2.6)}\\
Gender (\% Female) & 461 (46.0) & 518.0 (51.6)\\
\cellcolor{gray!6}{Age (\%)} & \cellcolor{gray!6}{} & \cellcolor{gray!6}{}\\

\indent $[50,60)$ & 372 (37.1) & 524.6 (52.3)\\
\cellcolor{gray!6}{\indent [60,70)} & \cellcolor{gray!6}{346 (34.5)} & \cellcolor{gray!6}{279.6 (27.9)}\\
\indent $[70,80)$ & 210 (20.9) & 158.1 (15.8)\\
\cellcolor{gray!6}{\indent [80,85)} & \cellcolor{gray!6}{75 (7.5)} & \cellcolor{gray!6}{40.6 (4.1)}\\
Education (\%) &  & \\

\cellcolor{gray!6}{\indent Less than High School} & \cellcolor{gray!6}{256 (25.5)} & \cellcolor{gray!6}{144.7 (14.4)}\\
\indent High School & 246 (24.5) & 266.3 (26.6)\\
\cellcolor{gray!6}{\indent College and Above} & \cellcolor{gray!6}{501 (50.0)} & \cellcolor{gray!6}{592.0 (59.0)}\\
Number of Alcoholic Drinks per Week (mean (SD)) & 2.87 (6.13) & 3.16 (6.31)\\
\cellcolor{gray!6}{Cigarette Smoking (\%)} & \cellcolor{gray!6}{} & \cellcolor{gray!6}{}\\

\indent Never & 464 (46.3) & 472.1 (47.1)\\
\cellcolor{gray!6}{\indent Former} & \cellcolor{gray!6}{377 (37.6)} & \cellcolor{gray!6}{371.2 (37.0)}\\
\indent Current & 162 (16.2) & 159.7 (15.9)\\
\cellcolor{gray!6}{Diabetes (\% Yes)} & \cellcolor{gray!6}{127 (12.7)} & \cellcolor{gray!6}{98.9 (9.9)}\\
Congestive Heart Failure (\% Yes) & 27 (2.7) & 22.9 (2.3)\\

\cellcolor{gray!6}{Coronary Heart Disease (\% Yes)} & \cellcolor{gray!6}{57 (5.7)} & \cellcolor{gray!6}{59.6 (5.9)}\\
Cancer (\% Yes) & 134 (13.4) & 137.5 (13.7)\\
\cellcolor{gray!6}{Stroke (\% Yes)} & \cellcolor{gray!6}{24 (2.4)} & \cellcolor{gray!6}{20.9 (2.1)}\\
HDL Cholesterol (mean (SD)) & 56.20 (16.58) & 56.82 (16.08)\\
\cellcolor{gray!6}{Total Cholesterol (mean (SD))} & \cellcolor{gray!6}{204.71 (41.57)} & \cellcolor{gray!6}{206.97 (40.66)}\\

Systolic Blood Pressure (mean (SD)) & 131.14 (20.54) & 129.16 (19.81)\\
\bottomrule
\end{longtable}


==> A comparison of functional principal component analysis methods with accelerometry applications/table_AUC.tex <==
\begin{table}[th]
    \caption{AUC scores for out-of-sample mortality prediction}
\label{tab:2}
\centering
\begin{tabular}[t]{lllll}
\toprule
Model & GFPCA & NARFD & PFPCA &Baseline (no FPCA scores)\\
\midrule
\cellcolor{gray!6}{AdaBoost} & \cellcolor{gray!6}{0.717} & \cellcolor{gray!6}{0.744} & \cellcolor{gray!6}{0.754}&
\cellcolor{gray!6}{0.729}\\
Logistic & 0.555 & 0.554 & 0.538 &0.555\\
\cellcolor{gray!6}{Random Forest} & \cellcolor{gray!6}{0.724} & \cellcolor{gray!6}{0.703} & \cellcolor{gray!6}{0.722}&
\cellcolor{gray!6}{0.733}\\
\bottomrule
\end{tabular}
\end{table}


==> A comparison of functional principal component analysis methods with accelerometry applications/table_coef1.tex <==

\begin{longtable}[t]{ll}
\caption{Coefficients table for logistic + PFPCA \\
*For categorical variable, the base level is given $0$ and $(0,0)$ as the coefficients and $95\%$ confidence intervals.}\\
\label{tab:coef1} \\
\toprule
 Variable & Coefficient (95 \% Confidence Interval) \\
\midrule
\cellcolor{gray!6}{Intercept} & \cellcolor{gray!6}{-6.769 (-16.924, 3.386)}\\
Number of Weekdays & -0.066 (-0.493, 0.361)\\
\cellcolor{gray!6}{Number of weekend} & \cellcolor{gray!6}{0.153 (-0.742, 1.048)}\\
Body Mass Index & -0.013 (-0.097, 0.071)\\
\cellcolor{gray!6}{Race} & \cellcolor{gray!6}{} \\
\indent White & 0 $(0,0)^*$  \\
\cellcolor{gray!6}{\indent Black} &\cellcolor{gray!6}{-0.012 (-0.918, 0.895)}\\
\indent Hispanic & -0.055 (-1.091, 0.981)\\
\cellcolor{gray!6}{\indent Other}  & \cellcolor{gray!6}{-14.02 (-14.987, -13.052)} \\
Gender & \\
\cellcolor{gray!6}{\indent Female}&  \cellcolor{gray!6}{-0.007 (-0.552, 0.537)}\\
\indent Male &   0 $(0,0)^*$  \\
\cellcolor{gray!6}{Age} & \cellcolor{gray!6}{0.107 (0.036, 0.178)} \\
Education  &    \\
\cellcolor{gray!6}{\indent Less than High School} & \cellcolor{gray!6}{$0 (0,0)^*$}  \\
\indent High School & 0.379 (-0.45, 1.208) \\
\cellcolor{gray!6}{\indent College and Above} & \cellcolor{gray!6}{-0.329 (-1.097, 0.44)} \\
Number of Alcoholic Drinks per Week  & 0.034 (-0.018, 0.085) \\
\cellcolor{gray!6}{Cigarette Smoking } & \cellcolor{gray!6}{}\\
\indent Never &   0 $(0,0)^*$  \\
\cellcolor{gray!6}{\indent Former} &\cellcolor{gray!6}{0.548 (-0.585, 1.681)}  \\
\indent Current & 0.74 (-0.086, 1.566)\\
\cellcolor{gray!6}{Has Diabetes} & \cellcolor{gray!6}{0.58 (-0.49, 1.65)} \\
Has Congestive Heart Failure & -0.018 (-1.808, 1.772)\\
\cellcolor{gray!6}{Has Coronary Heart Disease} & \cellcolor{gray!6}{-0.221 (-1.748, 1.306)}\\
Has Cancer & 0.611 (0.208, 1.014) \\
\cellcolor{gray!6}{Has Stroke} & \cellcolor{gray!6}{-0.364 (-2.228, 1.5)}\\

HDL Cholesterol  & -0.013 (-0.031, 0.004)\\
\cellcolor{gray!6}{Total Cholesterol} & \cellcolor{gray!6}-0.002 (-0.011, 0.006){}\\
Systolic Blood Pressure  &  0 (-0.016, 0.017)\\
\cellcolor{gray!6}{$2^{nd}$ score of Poisson FPCA} & \cellcolor{gray!6}{0.006 (-0.002, 0.015)}\\
$3^{rd}$ score of Poisson FPCA & -0.031 (-0.078, 0.016)\\
\cellcolor{gray!6}{$4^{th}$ score of Poisson FPCA} & \cellcolor{gray!6}{-0.015 (-0.046, 0.017)}\\

$5^{th}$ score of Poisson FPCA & 0.019 (-0.016, 0.055)\\
\cellcolor{gray!6}{$6^{th}$ score of Poisson FPCA} & \cellcolor{gray!6}{0.011 (-0.011, 0.032)}\\

\bottomrule
\end{longtable}

==> A comparison of functional principal component analysis methods with accelerometry applications/table_coef2.tex <==
\begin{table}[t]

\caption{Coefficents table for logistic + NARFD\\
*For categorical variable, the base level is given $0$ and $(0,0)$ as the coefficients and $95\%$ confidence intervals.}
\centering
\begin{tabular}[t]{ll}
\toprule
Variable & Coefficient(95\% Confidence Interval)\\
\midrule
\cellcolor{gray!6}{Intercept} & \cellcolor{gray!6}{-9.268 (-13.407, -5.129)}\\
Number of Weekdays  & -0.06 (-0.495, 0.374)\\
\cellcolor{gray!6}{Number of weekend} & \cellcolor{gray!6}{0.155 (-0.677, 0.987)}\\
Body Mass Index & -0.007 (-0.092, 0.078)\\
\cellcolor{gray!6}{Race} & \cellcolor{gray!6}{} \\
\indent White & 0 $(0,0)^*$  \\
\cellcolor{gray!6}{\indent Black} &\cellcolor{gray!6}{0.057 (-0.778, 0.893)}\\
\indent Hispanic & -0.009 (-1.027, 1.01)\\
\cellcolor{gray!6}{\indent Other}  & \cellcolor{gray!6}{-13.992 (-14.855, -13.129)}\\
Gender & \\
\cellcolor{gray!6}{\indent Female}&  \cellcolor{gray!6}{0.005 (-0.512, 0.522)}\\
\indent Male &   0 $(0,0)^*$  \\
\cellcolor{gray!6}{Age} & \cellcolor{gray!6}{0.107 (0.036, 0.178)}\\
Education  &    \\
\cellcolor{gray!6}{\indent Less than High School} &\cellcolor{gray!6}{$0 (0,0)^*$}  \\
\indent High School  & 0.394 (-0.404, 1.191)\\
\cellcolor{gray!6}{\indent College and Above}  & \cellcolor{gray!6}{-0.324 (-1.046, 0.399)}\\
Number of Alcoholic Drinks per Week  & 0.037 (-0.019, 0.092)\\
\cellcolor{gray!6}{Cigarette Smoking } & \cellcolor{gray!6}{}\\
\indent Never &   0 $(0,0)^*$  \\
\cellcolor{gray!6}{Former} & \cellcolor{gray!6}{0.558 (-0.586, 1.702)}\\
Current & 0.701 (-0.112, 1.515)\\
\cellcolor{gray!6}{Has Diabetes} & \cellcolor{gray!6}{0.556 (-0.535, 1.648)}\\
\addlinespace
Has Congestive Heart Failure & 0 (-1.838, 1.838)\\
\cellcolor{gray!6}{Has Coronary Heart Disease} & \cellcolor{gray!6}{-0.203 (-1.716, 1.311)}\\
CancerYes & 0.604 (0.182, 1.025)\\
\cellcolor{gray!6}{Has Stroke} & \cellcolor{gray!6}{-0.371 (-2.241, 1.499)}\\
HDL Cholesterol  & -0.013 (-0.031, 0.005)\\
\addlinespace
\cellcolor{gray!6}{Total Cholesterol} & \cellcolor{gray!6}{-0.003 (-0.012, 0.006)}\\
Systolic Blood Pressure & 0 (-0.017, 0.016)\\
\bottomrule
\end{tabular}
\end{table}


==> A comparison of functional principal component analysis methods with accelerometry applications/table_coef3.tex <==
\begin{table}[t]

\caption{Coefficents table for logistic + GFPCA \\
*For categorical variable, the base level is given $0$ and $(0,0)$ as the coefficients and $95\%$ confidence intervals.}
\centering
\begin{tabular}[t]{ll}
\toprule
Variable & Coefficient(95\% Confidence Interval)\\
\midrule
\cellcolor{gray!6}{Intercept} & \cellcolor{gray!6}{-8.634 (-12.826, -4.442)}\\
Number of Weekdays & -0.096 (-0.543, 0.351)\\
\cellcolor{gray!6}{Number of weekend} & \cellcolor{gray!6}{0.112 (-0.708, 0.932)}\\
Body Mass Index  & -0.013 (-0.097, 0.071)\\
\cellcolor{gray!6}{Race} & \cellcolor{gray!6}{} \\
\indent White & 0 $(0,0)^*$  \\
\cellcolor{gray!6}{\indent Black} & \cellcolor{gray!6}{0.098 (-0.78, 0.975)}\\
\indent Hispanic & 0.006 (-1.02, 1.033)\\
\cellcolor{gray!6}{\indent Other} & \cellcolor{gray!6}{-14.142 (-15.166, -13.119)}\\
Gender & \\
\cellcolor{gray!6}{\indent Female}& 0.081 (-0.505, 0.666)\\
\indent Male &   0 $(0,0)^*$  \\
\cellcolor{gray!6}{Age} & \cellcolor{gray!6}{0.103 (0.028, 0.177)}\\
Education  &    \\
\cellcolor{gray!6}{\indent Less than High School} &\cellcolor{gray!6}{$0 (0,0)^*$}  \\
\indent High School  & 0.411 (-0.403, 1.226)\\
\cellcolor{gray!6}{\indent College and Above} & \cellcolor{gray!6}{-0.302 (-1.031, 0.427)}\\
Number of Alcoholic Drinks per Week  & 0.036 (-0.021, 0.093)\\
\cellcolor{gray!6}{Cigarette Smoking } & \cellcolor{gray!6}{}\\
\indent Never &   0 $(0,0)^*$  \\
\cellcolor{gray!6}{\indent Former} & \cellcolor{gray!6}{0.553 (-0.571, 1.677)}\\
\indent Current  & 0.782 (-0.091, 1.655)\\
\cellcolor{gray!6}{Has Diabetes}& \cellcolor{gray!6}{0.523 (-0.604, 1.65)}\\
Has Congestive Heart Failure & -0.013 (-1.786, 1.76)\\
\cellcolor{gray!6}{Has Coronary Heart Disease} & \cellcolor{gray!6}{-0.17 (-1.733, 1.392)}\\
Has Cancer  & 0.6 (0.174, 1.026)\\
\cellcolor{gray!6}{Has Stroke} & \cellcolor{gray!6}{-0.5 (-2.342, 1.342)}\\
HDL Cholesterol  & -0.013 (-0.033, 0.006)\\
\cellcolor{gray!6}{Total Cholesterol} & \cellcolor{gray!6}{-0.003 (-0.012, 0.007)}\\
Systolic Blood Pressure & -0.001 (-0.018, 0.015)\\
\cellcolor{gray!6}{$4^{th}$ score of Gaussian FPCA} & \cellcolor{gray!6}{0.057 (0.006, 0.109)}\\
\bottomrule
\end{tabular}
\end{table}

